Network Architecture Search for Domain Adaptation

Deep networks have been used to learn transferable representations for domain adaptation. Existing deep domain adaptation methods systematically employ popular hand-crafted networks designed specifically for image-classification tasks, leading to sub-optimal domain adaptation performance. In this paper, we present Neural Architecture Search for Domain Adaptation (NASDA), a principle framework that leverages differentiable neural architecture search to derive the optimal network architecture for domain adaptation task. NASDA is designed with two novel training strategies: neural architecture search with multi-kernel Maximum Mean Discrepancy to derive the optimal architecture, and adversarial training between a feature generator and a batch of classifiers to consolidate the feature generator. We demonstrate experimentally that NASDA leads to state-of-the-art performance on several domain adaptation benchmarks.

==> Tables_Alg/exp_digits.tex <==
\begin{table}[!htbp]
  \vspace{0pt}
  \addtolength{\tabcolsep}{6pt}
  \centering 
  \caption{Accuracy (\%) on {Digits} for unsupervised domain adaptation }
  \label{table:more}
  \vspace{-5pt}
  \resizebox{0.8\textwidth}{!}{%
  \begin{tabular}{cccccc}
  	\toprule
    Method & MNIST $\rightarrow$ USPS & USPS $\rightarrow$ MNIST & SVHN $\rightarrow$ MNIST & Avg \\
    \midrule % non NAS method
    MMD  \\
    DANN & 77.1 & 73.0 & 71.1 &  & \\
    DSN & 91.3 & - & 82.7 &  & \\
    MCD~\cite{MCD_2018}  & 94.2 & 94.1 & 96.2 &  \\
    SRDA(RAN)~\cite{} \\
    CyCleGAN & 97.1 & 98.3 & 97.5 \\
    \midrule % NAS method
    NASNet & 98.4 & 99.0 & 98.8 & \\
    AmoebaNet &  & 98.98 & 91.5 &  & \\
    DARTS  & 98.1 &  &  &  &\\
    PDARTS  & 96.9 &   &  &  &  \\
    \textbf{NASDA}  &  98.0 & 97.76  & 98.6 &  \\
    \bottomrule
  \end{tabular}
  }
  \vspace{-13pt}
\end{table}

==> Tables_Alg/exp_synsig.tex <==
\begin{wraptable}{r}{0.4\textwidth}
% \begin{table}[t!]
  \addtolength{\tabcolsep}{3pt}
  
  \centering 
  \caption[width=0.2\textwidth]{Accuracy (\%) on {Traffic Signs}.}
  \label{tab_traffic}
%   \label{tab_exp}
%   \vspace{-5pt}
  \resizebox{0.4\textwidth}{!}{%
  \begin{tabular}{ccc}
  	\toprule
    Method & SYN Sign $\rightarrow$ GTSRB \\
    % GTRSB  $\rightarrow$ SYNSig & 
    % CIFAR $\rightarrow$ STL  &
    \midrule % non NAS method
     DAN~\cite{li2017mmd} &91.1\\
     DANN~\cite{DANN}  & 88.7 \\
     DSN~\cite{dsn} & 93.1   \\
     CORAL~\cite{sun2016deep} & 86.9 \\
     SRDA-RAN~\cite{srda}& 93.6 \\
    MCD~\cite{MCD_2018} & 94.2   \\
    ASSOC~\cite{ASSC} & 82.8 \\
    \midrule % NAS method
    \textbf{NASDA}  & 93.7 \\
    \bottomrule
  \end{tabular}
  }
  \vspace{-0.3cm}
%   \vspace{-13pt}
% \end{table}

\end{wraptable}

==> Tables_Alg/exps_all.tex <==
\begin{table}[t!]
  \vspace{0pt}
  \addtolength{\tabcolsep}{6pt}
  \centering 
  \caption{Accuracy (\%) on {Digits} and {STL$\rightarrow$CIFAR10} for unsupervised domain adaptation.}
  \label{tab_exp}
%   \vspace{-5pt}
  \resizebox{\textwidth}{!}{%
  \begin{tabular}{ccccc|cc}
  	\toprule
    Method & M $\rightarrow$ U & U $\rightarrow$ M & S $\rightarrow$ M & Avg(digits) & Method & STL $\rightarrow$ CIFAR10 \\
    % GTRSB  $\rightarrow$ SYNSig & 
    % CIFAR $\rightarrow$ STL  &
    \midrule % non NAS method
    DAN~\cite{li2017mmd}  & 81.1 & - & 71.1 & 76.1 & DRCN~\cite{ghifary2016deep}&58.7\\
    DANN~\cite{DANN} & 85.1 & 73.0 & 71.1 & 76.4 & DANN~\cite{DANN}  & 56.9  \\
    DSN~\cite{dsn} & $91.3^*$ & - & 82.7 & - & DWT~\cite{roy2019unsupervised} & 71.2  \\
    ADDA~\cite{adda} & $89.4^*$  & 90.1 & 76.0 & - & DCSE~\cite{wang2018domain} & 73.0 \\
    CoGAN~\cite{cogan} & $91.2^*$ & 89.1 & - & - & SE~\cite{french2017self} & 74.2\\
    
    MCD~\cite{MCD_2018}  & 94.2 & 94.1 & 96.2 & 94.8 & MCD~\cite{MCD_2018} & 69.2 \\ %https://arxiv.org/pdf/1909.05288v1.pdf
    G2A~\cite{g2a} & 95.0 & 90.8 & 92.4 &  92.7&  G2A~\cite{g2a} & 72.8\\
    SBADA-GAN~\cite{sbada} & 95.3 & 97.6 & 76.1 & 89.7 & VADA~\cite{shu2018dirt} & 73.5\\
    d-SNE~\cite{xu2019d} & \textbf{99.0} & 98.7 & 96.5 & \underline{98.1} & DIRT-T~\cite{shu2018dirt} & \underline{75.3}\\
    
    \midrule % NAS method
    \textbf{NASDA}  &  98.0 & \textbf{98.7}  & \textbf{98.6} & \textbf{98.4} &\textbf{NASDA} & \textbf{76.8} \\
    \bottomrule
  \end{tabular}
  }
%   \vspace{-13pt}
\end{table}

==> Tables_Alg/tab_param.tex <==
\begin{table}[!htbp]
  \vspace{0pt}
  \addtolength{\tabcolsep}{6pt}
  \centering 
  \caption{Architecture Statistics }
  \label{table:more}
  \vspace{-5pt}
  \resizebox{\textwidth}{!}{%
  \begin{tabular}{cccc}
  	\toprule
    Method &  & Params (M) & Search Cost (GPU days) & \\
    NASNet &  & 3.3  & 1,800 \\
    DARTS  &  & 3.3 & 1.5 \\
    PDARTS  &  & 3.4 & 0.3 \\
    \textbf{NASDA}  &  3.4 & \textbf{70.0} \\
    \bottomrule
  \end{tabular}
  }
  \vspace{-13pt}
\end{table}
